SkillMimicGen: Automated Demonstration Generation for Efficient Skill Learning and Deployment

Imitation learning from human demonstrations is an effective paradigm for robot manipulation, but acquiring large datasets is costly and resource-intensive, especially for long-horizon tasks. To address this issue, we propose SkillMimicGen (SkillGen), an automated system for generating demonstration datasets from a few human demos. SkillGen segments human demos into manipulation skills, adapts these skills to new contexts, and stitches them together through free-space transit and transfer motion. We also propose a Hybrid Skill Policy (HSP) framework for learning skill initiation, control, and termination components from SkillGen datasets, enabling skills to be sequenced using motion planning at test-time. We demonstrate that SkillGen greatly improves data generation and policy learning performance over a state-of-the-art data generation framework, resulting in the capability to produce data for large scene variations, including clutter, and agents that are on average 24% more successful. We demonstrate the efficacy of SkillGen by generating over 24K demonstrations across 18 task variants in simulation from just 60 human demonstrations, and training proficient, often near-perfect, HSP agents. Finally, we apply SkillGen to 3 real-world manipulation tasks and also demonstrate zero-shot sim-to-real transfer on a long-horizon assembly task. Videos, and more at https://skillgen.github.io.

==> 0-preamble.tex <==
\usepackage{marginnote}
\usepackage{graphics}
\usepackage[pdftex]{graphicx}
\usepackage{wrapfig}
\DeclareGraphicsExtensions{.pdf,.png,.jpg}

\usepackage[font={small}]{caption}
\usepackage{subcaption}
\usepackage[rightcaption]{sidecap}
\usepackage{pbox}

\usepackage{mathtools}
\usepackage{amsmath, amssymb, amscd}
\usepackage{ wasysym } %
\usepackage{amsfonts}
\usepackage{mathptmx} %
\usepackage{gensymb} 
\usepackage{nicefrac}       %

\DeclareMathAlphabet{\mathcal}{OMS}{lmsy}{m}{n}
\DeclareSymbolFont{largesymbols}{OMX}{cmex}{m}{n}
\usepackage{textcomp} %
\usepackage{dsfont}



\usepackage{array} %
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{booktabs}

\usepackage[
  separate-uncertainty = true,
  multi-part-units = repeat
]{siunitx}
\usepackage[T1]{fontenc} 
\usepackage[utf8]{inputenc}
\usepackage[english]{babel} %
\usepackage{units}
\usepackage{bm}
\usepackage{times} %
\usepackage{xspace}
\usepackage{flushend}%
\usepackage{csquotes}
\usepackage{makeidx}

\let\labelindent\relax
\usepackage{enumitem}

\usepackage{soul} %
\usepackage{subfiles} %
\usepackage[protrusion=true,expansion=true]{microtype}
\setlength{\emergencystretch}{3em}

\usepackage[yyyymmdd]{datetime}
\renewcommand{\dateseparator}{-}
\date{\protect\formatdate{1}{1}{2001}}

\usepackage{cite} %


\usepackage{url}

\usepackage{soul} %
\newcommand{\todohl}[1]{{[\hl{#1}]}}

\newcommand{\todo}[1]{\textcolor{red}{[#1]}}
\newcommand{\yuke}[1]{\textcolor{red}{[Yuke: #1]}}

\newcommand{\etal}{et al.~}
\newcommand{\tocite}[1]{%
\textcolor{red}{[cite:\ifthenelse{\equal{#1}{}}{}{#1}?]}
}

\newcommand{\ignore}[1]{}


\newcommand{\figlabel}[1]{\label{fig:#1}}
\newcommand{\figref}[1]{Figure\,\ref{fig:#1}}

\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Section\,\ref{sec:#1}}

\newcommand{\chlabel}[1]{\label{ch:#1}}
\newcommand{\chref}[1]{Chapter\,\ref{ch:#1}}

\newcommand{\tablabel}[1]{\label{tab:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}

\newcommand{\argmin}{\operatornamewithlimits{arg\ min}}
\newcommand{\argmax}{\operatornamewithlimits{arg\ max}}
\newcommand{\numshapes}{17 }
\newcommand{\analyticname}{Analytic }

\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
\newtheorem{definition}{Definition}
\newtheorem{problem}{Problem}
\newtheorem{property}{Property}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}

\newcommand{\versionString}{\textcolor{red}{draft-mode-[\today\ \currenttime]}}

\newcommand\roberto[1]{\sethlcolor{cyan}\hl{[R: #1]}}

\newcommand{\revision}[1]{#1}


==> 1-intro-june-4-2024.tex <==
\section{Introduction}
\label{sec:intro}

\input{figures/fig_pull}

Figure~\ref{fig:teaser}...

\ajay{Go back through, and add more citations to intro for more modern work, after filling out related work section.}

\ajay{HITL-TAMP needs to come first -- celebrate hybrid control paradigm, and its effectiveness, but too many assumptions at test-time, and data generation burden.}

Imitation learning from human demonstrations is an effective approach for training robots to perform different tasks. One popular technique is to have humans teleoperate robot arms to collect datasets for tasks of interest and then subsequently use the data to train robots to perform these tasks autonomously. Recent efforts have demonstrated that large, diverse datasets collected by teams of human demonstrators result in impressive and robust robot performance, and even allow the robots to generalize to different objects and tasks~\cite{TBD}. However, collecting large datasets in this way is costly and resource-intensive, often requiring several human operators, robots, and months of human effort. This data collection burden is a critical bottleneck for deploying imitation learning approaches. 

This need for data has motivated the development of data generation systems that seek to produce task demonstrations without human involvement. Some prior efforts employ an expert that observes privileged information to generate task demonstrations, but it can be difficult to apply such techniques to a wide range of tasks, compared to the tasks that humans are able to demonstrate through teleoperation. MimicGen~\cite{mandlekar2023mimicgen}, is a recently proposed data generation system that seeks to address this need. It uses a small number of human task demonstrations to automatically generate large datasets by splitting the source human data into object-centric sequences of end-effector targets, and then selectively transforming and sequencing such segments in new settings. 
\ajay{Consider adding a simple running task example that we can refer to, to compare MimicGen, HITL-TAMP, and MimicGen-MP}
While this is a simple and effective approach for data generation, there are some crucial limitations. 
\caelan{We likely want to avoid saying "MimicGen" and treat it as a competing approach rather than something we directly build on}

MimicGen uses a naive linear interpolation scheme during data generation to connect the end of one transformed object-centric human segment to another one. This approach is not aware of scene geometry, and consequently, this can result in data generation failures due to collisions between the robot and other objects in the scene. Furthermore, using longer (in time, not space) interpolation segments have been shown to be harmful to policy learning~\cite{mandlekar2023mimicgen}, resulting in the use of short interpolation segments with a small number of intermediate waypoints. However, this can lower the data generation success rate, since the end-effector controller might not be capable of accurately tracking waypoints that are far apart, and also be unsafe for real-world deployment. Consequently, the original MimicGen system has a fundamental tradeoff with respect to interpolation segments. On one hand, shorter segments are better for policy learning, but can result in lower data generation success rates and can be unsafe for real-world deployment, and on the other, longer segments are more suitable for real-world deployment and for ensuring better data generation throughput, but make policy learning more difficult. 
This motivates the question -- do we actually need to have an agent learn such interpolation segments, or can such segments be deferred to a non-learned component?
\caelan{This feels like we are just "changing the interpolation"}
\caelan{By shortening the skills, they also stay closer to the reference frame, so state aspects not covered by the reference frame are less likely to affect the demos}

Recent work has demonstrated the benefit of decomposing tasks into segments that are learned end-to-end with a trained agent, and segments that are carried out by non-learned components, such as a motion planner. In particular, HITL-TAMP~\cite{mandlekar2023human} established a paradigm where a Task and Motion Planner (TAMP)~\cite{garrett2021integrated} selectively asks a human for demonstrations (at train-time) or an agent to solve the task segment (at test-time), on specific parts of the task. HITL-TAMP showed that such TAMP-gated agents dramatically outperform their end-to-end counterparts by limiting agents to only be responsible for the most challenging, contact-rich pieces of each task. However, unlike MimicGen, HITL-TAMP still suffers from the burden of human operator data collection to collect large datasets. Furthermore, the use of TAMP at test-time can result in unfavorable assumptions on knowledge about the scene and task, compared to end-to-end approaches.
\caelan{Same comment as about MimicGen. We could also hide some of the detail in the related work.}

\ajay{Need to turn some of below into numbered contributions and also include specific numbers}

In this work, we seek to leverage the benefits of both approaches, by introducing~\sysName, an extension of the MimicGen system that employs a motion planner during data generation. This allows us to utilize a similar control decomposition to HITL-TAMP, embedded within the MimicGen data generation loop.
We learn proficient policies from data produced by~\sysName via a flexible learning framework that can leverage the motion planner at test-time, and that can integrate differing levels of assumptions at test-time.
\caelan{Need to expand on assumptions}
\sysName compares favorably to MimicGen by allowing data to be generated in more diverse settings, including scenes with clutter, by producing much more capable trained agents from the generated datasets, and by facilitating safe policy learning on real hardware, which was a significant limitation of original system. 
\caelan{The skills might still be unsafe, but otherwise, this is an advantage}
\sysName compares favorably to HITL-TAMP by dramatically reducing the operator data collection burden, and by reducing the assumptions needed for agent deployment, while retaining the core advantage of improved policy performance through a hybrid policy architecture.
\caelan{We need to discuss the hybrid policy with the about the same emphasis as the data generation}
\ajay{The hybrid policy is not as much of a novelty, e.g. see https://arxiv.org/abs/2306.17237, but we can place more emphasis on the learning, just not on equal footing}

\textbf{The primary contributions of this papers are:}
\begin{itemize}
    \item TBD
\end{itemize}

\caelan{We could possibly frame the data amplification as a global optimization/planning to best address the new problem. Could be viewed as a shooting method.}


==> A-object_transfer.tex <==
\section{Object Transfer}
\label{app:object_transfer}

TODO: stretch goal, object transfer and "all" transfer results for data generation and policy learning, another advantage over MimicGen


==> A-related.tex <==
\section{Full Related Work}
\label{app:related}

TODO


==> A-retired.tex <==
\section{Retired}


\noindent
References
\begin{itemize}
    \item \href{https://docs.google.com/spreadsheets/d/1XTUvfzL1Sji53rxqM8cMKrPTVb0S85LV6q0108NEYuc/edit?pli=1#gid=793424966}{Results Spreadsheet}
    \item \href{https://www.overleaf.com/project/645400e27cd52a49bc88cd64}{HITL-TAMP Overleaf}
    \item \href{https://www.overleaf.com/project/645400d042a7cf90ea1b4961}{MimicGen Overleaf}
    \item \href{https://nvidia-my.sharepoint.com/:p:/r/personal/amandlekar_nvidia_com/_layouts/15/Doc.aspx?sourcedoc=%
    \item \href{https://nvidia-my.sharepoint.com/:p:/r/personal/danfeix_nvidia_com/_layouts/15/Doc.aspx?sourcedoc=%
    \item \href{https://docs.google.com/spreadsheets/d/1XTUvfzL1Sji53rxqM8cMKrPTVb0S85LV6q0108NEYuc/edit?pli=1#gid=793424966}{Results Spreadsheet}
    \item \href{https://nvidia-my.sharepoint.com/:p:/r/personal/cgarrett_nvidia_com/_layouts/15/doc2.aspx?sourcedoc=%
    \item \href{https://drive.google.com/drive/u/2/folders/1tYojSTXFNr1AV02fk8vMcY_lnxTOsIF4}{qualitative\_videos}
\end{itemize}


\subsection{MimicGen}
\ajay{Move to Related Work, special section, delete the details, and just focus on outcomes of MimicGen not working well due to how it sequences motions linearly.}

Our method builds on the MimicGen data generation system. MimicGen takes a small {\em source} dataset of human demonstrations $\mathcal{D}_{\text{src}}$ collected on task $\mathcal{M}$ and produces a large generated dataset $\mathcal{D}$ on either the same task or a task variant (see above). 
\caelan{How do trajectories relate to actions?}

\textbf{Source Demonstration Parsing.} MimicGen first parses each trajectory in the source dataset $\tau \in \mathcal{D}_{\text{src}}$ into contiguous segments $\tau = (\tau_1, \tau_2, ..., \tau_{N_s})$, where each segment $\tau_i$ corresponds to an object-centric subtask $S_i(O_{S_i})$. Each segment is a sequence of target robot end effector poses in $\mathrm{SE}(3)$, %
$\tau_i = (T^{C_0}_W, T^{C_1}_W, ..., T^{C_K}_W)$ where $C_t$ is the controller target pose frame at timestep $t$, \caelan{Is there a reason both $C$ and $E$ are used here?}
$W$ is the world frame, and $K$ is the length of the segment. The end of each subtask in a demonstration $\tau$ can be detected using either an automated metric (for example, a successful object grasp or insertion) or manual human annotation.

\textbf{Demonstration Generation.} Next, MimicGen attempts to generate new task demonstrations through a trial-and-error process. 
\caelan{Rejection sampling?}
Given a new scene, MimicGen generates and executes a segment for each object-centric subtask in the task. This consists of the following key steps for each subtask $S_i(O_{S_i})$. First, a reference subtask segment $\tau_i$ from  $\mathcal{D}_{\text{src}}$ is chosen -- this can be a random selection or use heuristics. 
\caelan{In \sysName, we could sample several adaptations per task and take the best one}
Next, each target pose in $\tau_i$ is transformed according to the pose of object $O_{S_i}$ in the new scene $T^{O'_0}_W$, in order to preserve the relative poses between the target pose frame and the object frame at each timestep between the source demonstration segment and the new trajectory segment. This produces the transformed segment $\tau'_i = (T^{C'_0}_W, T^{C'_1}_W, ..., T^{C'_K}_W)$ where $T^{C'_t}_W = T^{O'_0}_{W}(T^{O_0}_{W})^{-1} T^{C_t}_W$~\cite{mandlekar2023mimicgen}. However, the first target pose of the transformed segment $T^{C'_0}_W$ could be far from the current robot end effector pose in the new scene $T^{E'_0}_W$. Thus, MimicGen adds an \textit{interpolation segment} at the start of $\tau'_i$, consisting of a sequence of 
$N_I$ target poses $(T^{I_1}_W, T^{I_2}_W, ..., T^{I_{N_I}}_W)$ that linearly interpolate between $T^{E'_0}_W$ and $T^{C'_0}_W$. 
\caelan{Was $E'$ defined?}
Finally, the segment $\tau'_i$ is executed by the robot controller. The steps above repeat for each subtask. After executing the segment for the final subtask, MimicGen checks for task success, and only keeps the demonstration if it was successful. The ratio between the number of successfully generated trajectories and the total number of attempts is the \textit{data generation rate}.

\caelan{Let's allow for flexibility in how the initial demonstrations are generated (human, HITL-TAMP, etc.). We can optionally say that we use HITL-TAMP as a detail.}

\subsection{Gated Control Policies}

\caelan{I think "Gated" is less relevant here. Ultimately, in the primary application, the learner decides the handoff locations. The use of polices in HITL-TAMP is mostly a bonus/ablation}

Instead of training a single monolithic agent that solves the entire manipulation task, gated-control policies opt to deploy a trained agent $\pi_{\theta}$ only during select parts of each task. They leverage a \textit{gating mechanism} to decide when the trained agent should act, and let another mechanism act during the remainder of each episode. For example, HITL-TAMP~\cite{mandlekar2023human} uses \textit{TAMP-gated} control policies, where a Task and Motion Planning (TAMP) system~\cite{garrett2021integrated} decides when to employ the trained agent. The rest of each episode is carried out by the TAMP system -- this allows the trained agent to only be responsible for contact-rich and low-tolerance segments of each manipulation task, while the TAMP system allows applying agents trained in this way to long-horizon manipulation. HITL-TAMP showed that such gated-control agents can enable effective contact-rich and long-horizon manipulation. However, the use of a TAMP system requires several assumptions -- including knowledge of when handoffs should take place between the TAMP system and the learned agent, and which pose targets the planner should reach before handing off control. In this work, introduce novel variants of gated-control policies (described in Sec.~\ref{sec:method}) that make use of a motion planner $\mathcal{M}$ instead of a full TAMP system. These agents are \textit{learning-gated} -- a trained network decides when the agent should act, and also where handoff should take place (e.g. which pose target the motion planner should reach before handoff).
\caelan{Move to Baselines}







\subsection{Brainstorming}

\noindent
\textbf{Caelan brainstorm:}
\begin{itemize}
    \item Task planning - LLM, state machine, behavior tree, etc.
    \item Two-level hierarchy
    \item Online vs offline execution
    \item Avoid using planning terminology
    \item Single neural network for each skill
    \item Condition skills on task vs skill
    \item Learn all skills simultaneously
    \item Single skill that's deployed in several contexts
    \item Deployment in HITL-TAMP (with and without learned constraints)
\end{itemize}

\textbf{LTAMP}
\begin{itemize}
    \item Initiation: GP learned
    \item Policy: GP learned parameterized
    \item Termination: fixed
\end{itemize}

\textbf{HITL-TAMP demonstration}
\begin{itemize}
    \item Initiation: memorized
    \item Policy: teleoperation
    \item Termination: engineered
\end{itemize}

\textbf{HITL-TAMP test}
\begin{itemize}
    \item Initiation: memorized
    \item Policy: NN visuomotor
    \item Termination: engineered
\end{itemize}

\textbf{\sysName demonstration}
\begin{itemize}
    \item Initiation: segmented
    \item Policy: replay
    \item Termination: segmented
\end{itemize}

\textbf{\sysName test}
\begin{itemize}
    \item Initiation: NN regressor
    \item Policy: NN visuomotor
    \item Termination: NN classifier
\end{itemize}

\textbf{MimicGen}
\begin{itemize}
    \item Policy: teleoperation/replay
\end{itemize}

\textbf{PerAct}
\begin{itemize}
    \item Policy: TBD
\end{itemize}


==> A-survey.tex <==
\section{Survey}

\ajay{Decide if we want to include this or not}

\begin{table}[h]
\begin{tabular}{@{}llll@{}}
\toprule
\textbf{Method} & \textbf{Initiation} & \textbf{Policy} & \textbf{Termination}\\
\midrule
Wang {\it et al.}~\cite{wang2021learning}    & Parametric: GP   & Parametric: GP  & Parametric: GP  \\
PerAct~\cite{shridhar2022peract}    & Keyframe: NN   & N/A  & N/A  \\
RVT~\cite{goyal2023rvt}    & Keyframe: NN   & N/A  & N/A  \\

MimicGen~\cite{mandlekar2023mimicgen}: Demo    & N/A   & Teleoperation  & N/A  \\
MimicGen~\cite{mandlekar2023mimicgen}: Gen    & N/A   & Adaptation  & N/A  \\
MimicGen~\cite{mandlekar2023mimicgen}: Test    & N/A   & BC: NN  & N/A  \\

HITL-TAMP~\cite{mandlekar2023human}: Data    & Memorized   & Teleoperation  & TAMP-gated  \\
HITL-TAMP~\cite{mandlekar2023human}: Test    & Memorized   & BC: NN  & TAMP-gated  \\

\underline{\sysName: Demo}    & Annotated   & Teleoperation  & Annotated  \\
\underline{\sysName: Gen}    & Memorized   & Adaptation  & Memorized  \\
\underline{\sysName: Test}    & Keyframe: NN   & BC: NN  & Learned: NN  \\
\bottomrule
\end{tabular}
\caption{\caelan{WIP} - A table surveying the implementation of the 3 skill components across prior work and \sysName. Abbreviations: Gaussian Process (GP), Neural Network (NN), Behavior Cloning (BC).}\label{table:skill}%
\end{table}
\caelan{TODO: Include other methods (like Hydra)?}

\caelan{Optional, but a useful brainstorming exercise:} Table~\ref{table:skill} interprets \sysName as well as prior works using the skill abstraction according to how their initiation, policy, and termination conditions are implemented, if present.
Wang {\it et al.}~\cite{wang2021learning} consider skills where the sequence of states and actions are manually parameterized and the parameters are learned using tabular Gaussian Processes.
PerAct~\cite{shridhar2022peract} and RVT~\cite{goyal2023rvt} both predict keyframes that can be interpreted as instantaneous skills.
MimicGen~\cite{mandlekar2023mimicgen} does not consider skills and thus the initiation and termination conditions are not applicable.
HITL-TAMP~\cite{mandlekar2023human} memorizes the initiation set in the form of constraints and implements the termination condition using a TAMP-gated test on the state.
In contrast, \sysName uses skill adaptation at data generation time and learns each skill component at deployment time.

